A Multi-Loss Strategy for Vehicle Trajectory Prediction: Combining Off-Road, Diversity, and Directional Consistency Losses

Trajectory prediction is essential for the safety and efficiency of planning in autonomous vehicles. However, current models often fail to fully capture complex traffic rules and the complete range of potential vehicle movements. Addressing these limitations, this study introduces three novel loss functions: Offroad Loss, Direction Consistency Error, and Diversity Loss. These functions are designed to keep predicted paths within driving area boundaries, aligned with traffic directions, and cover a wider variety of plausible driving scenarios. As all prediction modes should adhere to road rules and conditions, this work overcomes the shortcomings of traditional "winner takes all" training methods by applying the loss functions to all prediction modes. These loss functions not only improve model training but can also serve as metrics for evaluating the realism and diversity of trajectory predictions. Extensive validation on the nuScenes and Argoverse 2 datasets with leading baseline models demonstrates that our approach not only maintains accuracy but significantly improves safety and robustness, reducing offroad errors on average by 47% on original and by 37% on attacked scenes. This work sets a new benchmark for trajectory prediction in autonomous driving, offering substantial improvements in navigating complex environments. Our code is available at https://github.com/vita-epfl/stay-on-track .

==> sections/intro.tex <==
% \skeleton{Introduce trajectory prediction problem and state that it has been advanced a lot in the past years.}
Trajectory prediction plays a crucial role in autonomous systems, particularly in enhancing the safety and reliability of self-driving vehicles. In recent years, significant progress has been made in this field, with advanced models increasingly capable of anticipating the movements of dynamic agents in complex environments. Despite these advancements, current models still face challenges in critical areas such as scene understanding and the accurate prediction of all possible trajectory modes.

% \skeleton{However they have shortcomings in certain areas such as scene understanding and properly predicting all possible modes. For example, as shown in the pull figure, even state-of-the-art prediction models suffer from problems such as going off-road or opposite the flow of the traffic, and missing prediction modes.}
Despite recent advancements, many existing trajectory prediction models still lack a deep understanding of the scene, which is critical for accurate and safe predictions. This limitation is highlighted by Bahari et al., who demonstrate that models struggle when faced with natural scene changes, such as injecting a new turn in the road ahead of the ego vehicle. These perturbations disrupt model performance and expose their inability to fully comprehend complex environments, especially in scenarios that require understanding road layouts, traffic dynamics, and predicting various possible modes — such as navigating different turns or exits in a roundabout — where incorrect predictions could pose a significant safety risk for downstream path planning modules relying on these predictions.

% \skeleton{In this work, we propose three loss functions to overcome these challenges and add more inductive bias to the models. They include Offroad, Direction Consistency Error, and Diversity.}
To address the above challenges, this work introduces three novel loss functions designed to infuse additional inductive biases into trajectory prediction models. The proposed loss functions — Offroad Loss, Direction Consistency Error, and Diversity Loss — aim to enhance the model’s understanding of the scene, improve compliance with traffic rules, and promote prediction diversity, respectively.

% \skeleton{Our first loss, the Offroad Loss penalizes predictions that deviate from drivable areas, with penalties proportional to the distance from these areas. This ensures }
The Offroad Loss penalizes predictions that deviate from
drivable areas, with penalties proportional to the distance
from these areas. This approach builds on previous work
by Messaoud et al., who implemented a similar loss using
rasterized drivable area masks in the nuScenes dataset. How-
ever, as the field evolves towards using vectorized formats
for maps due to their efficiency and compact representation,
we have developed a vectorized version of the Offroad Loss,
implemented across three prominent datasets: nuScenes, Ar-
goverse 2, and Waymo.

% \skeleton{The second loss function we propose is called Direction Consistency Error. Similar to the first loss, this one also tries to teach the model to predict in the correct direction of the traffic in the scene. Simply put, this loss function calculates the 2D and angular distance between prediction points and centerline points in the scene. Therefore it penalizes predictions for which there is no close centerline with similar direction.}
The second proposed loss, Direction Consistency Error, further enhances scene understanding by aligning predictions with the correct traffic direction. This loss function penalizes predictions that do not align closely with the appropriate centerline directions. This ensures that predicted trajectories not only stay within drivable boundaries but also respect the natural flow of traffic.

% \skeleton{Finally, we also introduce diversity loss, which tries to encourage model to have more diverse set of predictions to cover all different possibilities, but as long as they make sense. To this end, we first remove the predictions that went offroad, and the calculate the sum of pairwise distance between the endpoints of the remaining predictions. It is essential to remove offroads in order not to artificially increase the diversity, rather to do it in a natural way. }
Finally, the Diversity Loss encourages the model to generate a varied set of predictions that encompass all plausible outcomes, provided they are reasonable. This is achieved by first filtering out predictions that violate scene constraints, followed by calculating the diversity of the remaining predictions. The filtering step is crucial to avoid artificially inflating diversity through implausible trajectories, ensuring that the model’s predictions remain both realistic and varied.

% \skeleton{Through many experiments on two state of the art baseline and on the three mentioned datasets, we investigate the effect of the proposed loss functions and their contribution to a safer prediction model, without a sacrifice in prediction accuracy.}
Through extensive experiments on two state-of-the-art baseline models across the nuScenes, Argoverse 2, and Waymo datasets, we evaluate the impact of the proposed loss functions. Our results demonstrate that these losses contribute to a more robust and safer trajectory prediction model without compromising prediction accuracy.

\begin{figure}[t]
  % \vspace{-20pt}
  \centering
  \includegraphics[width=0.7\linewidth]{figures/pull_figure.pdf}
  \caption{Visualization of a trajectory prediction scene, with predictions of a state-of-the-art trajectory prediction model. We can observe that some predictions are going off-road, and then entering a region where the traffic direction is opposite the predictions. Additionally, the model has not foreseen other behaviors in the intersection, such as continuing straight or turning left. We introduce loss functions to mitigate these undesirable predictions.}
   \label{fig:pull}
\end{figure}

==> sections/intro2.tex <==
% \skeleton{Introduce vehicle trajectory prediction problem and state that it has been advanced a lot in the past years.}
Vehicle trajectory prediction is an essential component of autonomous driving systems, ensuring safety and efficiency in dynamic environments. This field has seen significant advancements in recent years, driven by innovations in machine learning techniques and the availability of rich datasets. An intrinsic aspect of this prediction task is its multimodal nature, stemming from the fundamental uncertainty tied to drivers' intentions, driving styles, and other variable factors.

% \skeleton{Talk about the uncertainty in the prediction problem, and that as a result, we let the models to predict $K$ different trajectories for a single scenario to account for multiple possible futures. You can use an example to describe it better.}
Recognizing the inherent variability in human driving behavior, benchmarks in this field support models that can forecast multiple potential future trajectories for a single scenario. This multimodal approach is critical for capturing the range of possible outcomes that might occur in real-world situations. For instance, at an intersection, a predictive model may need to consider several feasible trajectories for a vehicle, such as turning left, continuing straight, or stopping due to traffic, each conditioned on different but equally plausible sets of assumptions about future driving behavior.

% \skeleton{Then say that the way people usually train their prediction models is by minimizing the prediction error on the closest prediction to ground truth where the winner takes all the gradient and the other predictions are not updated. This means different modes of the prediction could have suboptimal performance, specially the more rare ones.}
Traditionally, these prediction models are trained by minimizing the error of the predicted trajectory closest to the ground truth, a method known as the \textit{best-of-many} approach. This training strategy often results in the majority of the learning signal being concentrated on the most frequent or probable outcomes, potentially neglecting less common but equally plausible trajectories. As a result, the performance of these rarer prediction modes could be suboptimal, limiting the model’s effectiveness in diverse driving conditions.

% \skeleton{In this work, we propose three auxiliary loss functions that try to add scene compliance knowledge to all prediction modes of the model. They include Offroad, Direction Consistency Error, and Diversity.}
In response to these challenges, our work introduces three innovative auxiliary loss functions aimed at improving the fidelity and utility of multi-modal trajectory predictions. The proposed loss functions — Offroad Loss, Direction Consistency Error, and Diversity Loss — are designed to embed crucial scene compliance knowledge directly into the learning process of the prediction models. Each function specifically targets different aspects of prediction relevance and plausibility, ensuring that all potential outcomes generated by the model are not only diverse but also accurately reflect the real-world constraints and behaviors observed in vehicular dynamics.

% \skeleton{Our first loss penalizes predictions that go offroad, proportional to how distant they are from the drivable area. Messaoud et al have previously proposed a similar loss function for nuscenes dataset, where they calculated the distance of the predictions to some descreete rasterized drivable area mask. However the trend in the field has been towards using vectorized format for map instead of the rasterized ones. The reason is it is a more efficient and compact way of representing the model. We have implemented a vectorized version of offroad for the three most used datasets, nuScenes, argoverse 2, and waymo.}
The Offroad Loss penalizes predictions that deviate from drivable areas, with penalties proportional to the distance from these areas. This approach builds on previous work by Messaoud et al., who implemented a similar loss using rasterized drivable area masks in the nuScenes dataset. However, as the field evolves towards using vectorized formats for maps due to their efficiency and compact representation, we have developed a vectorized version of the Offroad Loss, implemented across three prominent datasets: nuScenes, Argoverse 2, and Waymo.

% \skeleton{The second loss function we propose is called Direction Consistency Error. Similar to the first loss, this one also tries to teach the model to predict in the correct direction of the traffic in the scene. Simply put, this loss function calculates the 2D and angular distance between prediction points and centerline points in the scene. Therefore it penalizes predictions for which there is no close centerline with similar direction.}
The second proposed loss, Direction Consistency Error, further enhances scene understanding by aligning predictions with the correct traffic direction. This loss function penalizes predictions that do not align closely with the appropriate centerline directions. This ensures that predicted trajectories not only stay within drivable boundaries but also respect the natural flow of traffic.

% \skeleton{Finally, we also introduce diversity loss, which tries to encourage model to have more diverse set of predictions to cover all different possibilities, but as long as they make sense. To this end, we first remove the predictions that went offroad, and the calculate the sum of pairwise distance between the endpoints of the remaining predictions. It is essential to remove offroads in order not to artificially increase the diversity, rather to do it in a natural way. }
Finally, the Diversity Loss encourages the model to generate a varied set of predictions that encompass all plausible outcomes, provided they are reasonable. This is achieved by first filtering out predictions that violate scene constraints, followed by calculating diversity of the remaining predictions. The filtering step is crucial to avoid artificially inflating diversity through implausible trajectories, ensuring that the model’s predictions remain both realistic and varied.

% \skeleton{Through many experiments on two state of the art baseline and on the three mentioned datasets, we investigate the effect of the proposed loss functions and their contribution to a safer prediction model, without a sacrifice in prediction accuracy.}
Through extensive experiments on two state-of-the-art baseline models across the nuScenes, Argoverse 2, and Waymo datasets, we evaluate the impact of the proposed loss functions. Our results demonstrate that these losses contribute to a more robust and safer trajectory prediction model without compromising prediction accuracy.

